WoLFRaM: Enhancing Wear-Leveling and Fault Tolerance in Resistive Memories using Programmable Address Decoders

Resistive memories have limited lifetime caused by limited write endurance and highly non-uniform write access patterns. Two main techniques to mitigate endurance-related memory failures are 1) wear-leveling, to evenly distribute the writes across the entire memory, and 2) fault tolerance, to correct memory cell failures. However, one of the main open challenges in extending the lifetime of existing resistive memories is to make both techniques work together seamlessly and efficiently. To address this challenge, we propose WoLFRaM, a new mechanism that combines both wear-leveling and fault tolerance techniques at low cost by using a programmable resistive address decoder (PRAD). The key idea of WoLFRaM is to use PRAD for implementing 1) a new efficient wear-leveling mechanism that remaps write accesses to random physical locations on the fly, and 2) a new efficient fault tolerance mechanism that recovers from faults by remapping failed memory blocks to available physical locations. Our evaluations show that, for a Phase Change Memory (PCM) based system with cell endurance of 108 writes, WoLFRaM increases the memory lifetime by 68% compared to a baseline that implements the best state-of-the-art wear-leveling and fault correction mechanisms. WoLFRaM's average / worst-case performance and energy overheads are 0.51% / 3.8% and 0.47% / 2.1% respectively.

==> 05_implementation.tex <==
%!TEX root =  main.tex
%\section{\mechanism{} Architecture and Implementation}
\section{\mechanism{} Controller}
\label{sec:Implementation}

The following sub-sections provide a detailed explanation of the in-memory \mechanism{} controller. 
Similar \lois{to previous works~\cite{seong2010security}, \mechanism{} implements a simple wear-leveling and fault tolerance controller at each memory bank.} \todo{Describe the advantages of doing this}

\mechanism{} remaps write addresses across a single bank. Each bank in the memory system has a separate \mechanism{} controller which controls the swap operation within the bank. To ensure proper functioning of the memory, the memory controller and the \mechanism{}c are tightly synchronized \todo{What this means exactly?}. 

\lois{The \mechanism{} controller also incorporates a random number generator to generate random numbers that trigger the swapping mechanism probabilistically.}\todo{Should we mention something about the overhead?}

\vspace{5pt}\noindent\textbf{{Memory Commands.}}
\mechanism{} \lois{does \emph{not} require new memory commands in the standard to perform the swap operation in-memory. Instead, the ACT and PRE commands (see Section~\ref{sec:resistive_memory_operation}) issued by the \mechanism{} are reinterpreted to operate in the SB instead of the RB.} 




